Keeping Deep Learning Models in Check: A History-Based Approach to Mitigate Overfitting

In software engineering, deep learning models are increasingly deployed for critical tasks such as bug detection and code review. However, overfitting remains a challenge that affects the quality, reliability, and trustworthiness of software systems that utilize deep learning models. Overfitting can be (1) prevented (e.g., using dropout or early stopping) or (2) detected in a trained model (e.g., using correlation-based approaches). Both overfitting detection and prevention approaches that are currently used have constraints (e.g., requiring modification of the model structure, and high computing resources). In this paper, we propose a simple, yet powerful approach that can both detect and prevent overfitting based on the training history (i.e., validation losses). Our approach first trains a time series classifier on training histories of overfit models. This classifier is then used to detect if a trained model is overfit. In addition, our trained classifier can be used to prevent overfitting by identifying the optimal point to stop a model's training. We evaluate our approach on its ability to identify and prevent overfitting in real-world samples. We compare our approach against correlation-based detection approaches and the most commonly used prevention approach (i.e., early stopping). Our approach achieves an F1 score of 0.91 which is at least 5% higher than the current best-performing non-intrusive overfitting detection approach. Furthermore, our approach can stop training to avoid overfitting at least 32% of the times earlier than early stopping and has the same or a better rate of returning the best model.

==> sections/ack.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
% \begin{acks}
% \section*{Acknowledgment}
% The work described in this paper has been supported by the ECE-Huawei Research Initiative (HERI) at the University of Alberta.
% \end{acks}


==> sections/guidelines.tex <==
\section{Guidelines}\label{sec:guidelines}

\textit{For Researchers:}
We highlight the importance of training history as a valuable asset for both detecting and preventing overfitting. Our study demonstrates the efficacy of using time series classifiers~(particularly KNN-DTW) for detecting overfitting with an F1 score of 0.91~(as detailed in Section~\ref{sec:rq1}). If post-hoc overfitting detection is required for your research, we advocate adopting our approach to validate the trained models. Although this approach incurs computational overhead, it is generally feasible since overfitting detection is executed only once after training is complete. For future work, we encourage exploration of optimization strategies to reduce the computational intensity of time series classifiers. Our replication package~\citep{replication_package} and experimental insights serve as a robust foundation for advancing research in this area.


\textit{For Practitioners:}
Our approach which uses KNN-DTW with a rolling window can stop training significantly earlier than traditional early stopping methods without sacrificing the model's performance~(see Section~\ref{sec:rq2}). This approach can be easily adapted into the existing codebase and is compatible with other overfitting prevention methods, such as dropout and regularization. The code changes required for integrating our method are minimal, making it broadly applicable across various use cases. Furthermore, our overfitting detection approach can be integrated into existing machine learning pipelines to ensure the quality of trained models. 

TODO: 
1. For DL frameworks, they can use our approach and keep envolving to improve the performance.
2. Move this section to conclusion section, maybe rename it as Implications and Conclusion



==> tabs/avg_cls_acc_error.tex <==
\begin{table}[tbhp]
\small
\centering
\caption{Results of the average classification accuracy of obtained models in the real-world dataset using overfitting prevention methods based on zero-one validation loss curves. (ES: early stopping; ES-SC: early stopping with smoothed curves; OPT: optimal classification accuracy)}
\label{tab:avg_cls_acc_error}
\begin{tabular}{rrrrrrrrrr}
\toprule
Ws. & BOSSVS & HMM-GMM & KNN-DTW & SAX-VSM & TSBF  & TSF   & ES    & ES-SC & OPT                    \\ \midrule
20  & 0.415  & 0.354   & 0.417   & 0.371   & 0.377 & 0.396 & 0.395 & 0.394 &  \multirow{5}{*}{0.434} \\
40  & 0.428  & 0.374   & 0.431   & 0.375   & 0.387 & 0.401 & 0.426 & 0.426 &                        \\
60  & 0.429  & 0.384   & 0.433   & 0.384   & 0.394 & 0.407 & 0.433 & 0.433 &                        \\
80  & 0.430  & 0.387   & 0.434   & 0.389   & 0.415 & 0.432 & 0.433 & 0.433 &                        \\
100 & 0.431  & 0.406   & 0.434   & 0.394   & 0.424 & 0.434 & 0.433 & 0.434 &                       \\ \bottomrule
\end{tabular}
\end{table}

==> tabs/early_stopping_patiences.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[tbhp]
\centering
\caption{Different values of patience for early stopping }
\label{tab:early_stopping_patience}
\begin{tabular}{@{}rrrr@{}}
\toprule
Patience & Correct Rate & Median diff btw opt & Median diff btw best and stop \\ \midrule
5        & 0.453461     & 405.0            & 5.0                    \\
10       & 0.594272     & 312.0            & 10.0                   \\
15       & 0.675418     & 273.5            & 15.0                   \\
20       & 0.723150     & 265.0            & 20.0                   \\
25       & 0.761337     & 260.0            & 25.0                   \\
30       & 0.782816     & 268.0            & 30.0                   \\
35       & 0.813842     & 284.5            & 35.0                   \\
40       & 0.835322     & 289.0            & 40.0                   \\
45       & 0.849642     & 310.0            & 45.0                   \\
50       & 0.861575     & 292.5            & 50.0                   \\
55       & 0.871122     & 292.5            & 55.0                   \\
60       & 0.887828     & 317.0            & 60.0                   \\
65       & 0.904535     & 379.0            & 65.0                   \\
70       & 0.911695     & 387.0            & 70.0                   \\
75       & 0.923628     & 397.0            & 75.0                   \\
80       & 0.930788     & 407.0            & 80.0                   \\
85       & 0.930788     & 407.0            & 85.0                   \\
90       & 0.937947     & 397.0            & 90.0                   \\
95       & 0.940334     & 407.0            & 95.0                   \\
100      & 0.940334     & 407.0            & 100.0                  \\
105      & 0.942721     & 419.5            & 105.0                  \\
110      & 0.942721     & 419.5            & 110.0                  \\
115      & 0.945107     & 432.0            & 115.0                  \\
120      & 0.949881     & 462.0            & 120.0                  \\
125      & 0.949881     & 462.0            & 125.0                  \\
130      & 0.952267     & 492.0            & 130.0                  \\
135      & 0.954654     & 522.0            & 135.0                  \\
140      & 0.954654     & 522.0            & 140.0                  \\
145      & 0.959427     & 522.0            & 145.0                  \\
150      & 0.964200     & 478.0            & 150.0                  \\
155      & 0.968974     & 432.0            & 155.0                  \\
160      & 0.971360     & 419.5            & 160.0                  \\
165      & 0.971360     & 419.5            & 165.0                  \\
170      & 0.973747     & 432.0            & 170.0                  \\
175      & 0.973747     & 432.0            & 175.0                  \\
180      & 0.973747     & 432.0            & 180.0                  \\
185      & 0.973747     & 432.0            & 185.0                  \\
190      & 0.973747     & 432.0            & 190.0                  \\
195      & 0.976134     & 553.0            & 195.0                  \\ \bottomrule
\end{tabular}
\end{table}

==> tabs/es_smooth.tex <==

\begin{table*}[t]
\centering
\caption{Results of early stopping based on the smoothed validation loss curves.}
\label{tab:es_smooth}
\begin{tabular}{lrrr|lrrr}
\toprule
Patience &
  \begin{tabular}[c]{@{}r@{}}Smooth \\ epochs\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Optimum\\ rate\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Median\\ delay\end{tabular} &
  Patience &
  \begin{tabular}[c]{@{}r@{}}Smooth \\ epochs\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Optimum\\ rate\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Median\\ delay\end{tabular} \\ \midrule
\multirow{4}{*}{20} & 0  & 0.48 & 20.0 & \multirow{4}{*}{60} & 0  & 0.90 & 60.0 \\
                    & 5  & 0.38 & 20.0 &                     & 5  & 0.93 & 61.0 \\
                    & 10 & 0.40 & 20.0 &                     & 10 & 0.93 & 62.0 \\
                    & 15 & 0.55 & 22.0 &                     & 15 & 0.90 & 62.0 \\ \midrule
\multirow{4}{*}{40} & 0  & 0.83 & 40.0 & \multirow{4}{*}{80} & 0  & 0.98 & 80.0 \\
                    & 5  & 0.85 & 42.0 &                     & 5  & 0.98 & 81.0 \\
                    & 10 & 0.83 & 43.5 &                     & 10 & 0.98 & 82.0 \\
                    & 15 & 0.88 & 44.5 &                     & 15 & 0.90 & 81.5 \\ \bottomrule
\end{tabular}
\end{table*}


==> tabs/evaluation_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tbhp]
\centering
\caption{Results of overfitting detection methods in the training and real-world datasets. (Prec: precision; Rec: recall; F-s: F-score; Avg F-s: macro average F-score)}
\label{tab:evaluation_res}
% \begin{tabular}{llrrrlllllrrrlllllrll}
% \hline
% \multicolumn{2}{l}{\multirow{3}{*}{Detection method}}                                            & \multicolumn{7}{c}{Non-overfitting}                                                                               &  & \multicolumn{7}{c}{Overfitting}                                                                                   &  & \multicolumn{3}{c}{Avg F-s}                                                                                              \\ \cline{3-9} \cline{11-17} \cline{19-21} 
% \multicolumn{2}{l}{}                                                                             & \multicolumn{3}{c}{Training} &  & \multicolumn{3}{c}{Real world}                                                  &  & \multicolumn{3}{c}{Training} &  & \multicolumn{3}{c}{Real world}                                                  &  & \multicolumn{1}{l}{\multirow{2}{*}{Training}} &  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Real\\ world\end{tabular}} \\
% \multicolumn{2}{l}{}                                                                             & Prec.    & Rec.    & F-s.    &  & \multicolumn{1}{r}{Prec.} & \multicolumn{1}{r}{Rec.} & \multicolumn{1}{r}{F-s.} &  & Prec.    & Rec.    & F-s.    &  & \multicolumn{1}{r}{Prec.} & \multicolumn{1}{r}{Rec.} & \multicolumn{1}{r}{F-s.} &  & \multicolumn{1}{l}{}                          &  &                                                                       \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Correlation\\ based\end{tabular}}          & Spearman & 0.67     & 0.73    & 0.70    &  &                           &                          &                          &  & 0.86     & 0.86    & 0.88    &  &                           &                          &                          &  & 0.79                                          &  &                                                                       \\
%                                                                                       & Pearson  & 1.00     & 0.55    & 0.71    &  &                           &                          &                          &  & 0.85     & 1.00    & 0.92    &  &                           &                          &                          &  & 0.81                                          &  &                                                                       \\
%                                                                                       & Autocorr & 1.00     & 0.73    & 0.84    &  &                           &                          &                          &  & 0.91     & 1.00    & 0.95    &  &                           &                          &                          &  & 0.90                                          &  &                                                                       \\ \hline
% PV                                                                                    & PV       & -        & -       & -       &  &                           &                          &                          &  & -        & -       & -       &  &                           &                          &                          &  & -                                             &  &                                                                       \\ \hline
% \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Time \\ series \\ classifier\end{tabular}} & KNN-DTW  & 0.79     & 1.00    & 0.88    &  &                           &                          &                          &  & 1.00     & 0.90    & 0.95    &  &                           &                          &                          &  & 0.91                                          &  &                                                                       \\
%                                                                                       & HMM      & 0.83     & 0.91    & 0.87    &  &                           &                          &                          &  & 0.96     & 0.93    & 0.95    &  &                           &                          &                          &  & 0.91                                          &  &                                                                       \\
%                                                                                       & TSF      & 0.77     & 0.91    & 0.83    &  &                           &                          &                          &  & 0.96     & 0.90    & 0.93    &  &                           &                          &                          &  & 0.88                                          &  &                                                                       \\
%                                                                                       & TSBF     & 0.67     & 0.91    & 0.77    &  &                           &                          &                          &  & 0.96     & 0.83    & 0.89    &  &                           &                          &                          &  & 0.83                                          &  &                                                                       \\
%                                                                                       & BOSSVS   & 0.83     & 0.91    & 0.87    &  &                           &                          &                          &  & 0.96     & 0.93    & 0.95    &  &                           &                          &                          &  & 0.91                                          &  &                                                                       \\
%                                                                                       & SAX-VSM  & 0.27     & 0.64    & 0.38    &  &                           &                          &                          &  & 0.71     & 0.34    & 0.47    &  &                           &                          &                          &  & 0.42                                          &  &                                                                       \\ \hline
% \end{tabular}
\begin{tabular}{llrrrllllrlrrrlllll}
\hline
\multicolumn{2}{l}{\multirow{3}{*}{Detection method}}                                                              & \multicolumn{8}{c}{Synthetic dataset}                                                                                                                                                          &  & \multicolumn{8}{c}{Real-world dataset}                                                                                                                                                                          \\ \cline{3-10} \cline{12-19} 
\multicolumn{2}{l}{}                                                                                               & \multicolumn{3}{c}{Non-overfitting} &  & \multicolumn{3}{c}{Overfitting}                                                & \multirow{2}{*}{\begin{tabular}[c]{@{}r@{}}Avg \\ F-s\end{tabular}} &  & \multicolumn{3}{c}{Non-overfitting} &  & \multicolumn{3}{c}{Overfitting}                                              & \multicolumn{1}{r}{\multirow{2}{*}{\begin{tabular}[c]{@{}r@{}}Avg \\ F-s\end{tabular}}} \\ \cline{3-5} \cline{7-9} \cline{12-14} \cline{16-18}
\multicolumn{2}{l}{}                                                                                               & Prec       & Rec        & F-s       &  & \multicolumn{1}{r}{Prec} & \multicolumn{1}{r}{Rec}  & \multicolumn{1}{r}{F-s}  &                                                                     &  & Prec       & Rec        & F-s       &  & \multicolumn{1}{r}{Prec} & \multicolumn{1}{r}{Rec} & \multicolumn{1}{r}{F-s} & \multicolumn{1}{r}{}                                                                    \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Correlation\\ based\end{tabular}}                            & Spearman & 0.99       & 1.00       & 0.99      &  & 0.95                     & 0.89                     & 0.92                     & 0.95                                                                &  & 0.67       & 0.73       & 0.70      &  & 0.89                     & 0.86                    & 0.88                    & 0.79                                                                                    \\
                                                                                                        & Pearson  & 0.99       & 0.97       & 0.98      &  & 0.79                     & 0.93                     & 0.85                     & 0.92                                                                &  & 1.00       & 0.55       & 0.71      &  & 0.85                     & 1.00                    & 0.92                    & 0.81                                                                                    \\
                                                                                                        & Autocorr & 0.97       & 0.94       & 0.95      &  & 0.59                     & 0.73                     & 0.65                     & 0.80                                                                &  & 1.00       & 0.46       & 0.63      &  & 0.83                     & 1.00                    & 0.91                    & 0.77                                                                                    \\ \hline
PV                                                                                                      & PV       & 0.89       & 0.85       & 0.87      &  & 0.07                     & 0.09                     & 0.08                     & 0.47                                                                &  & -          & -          & -         &  & \multicolumn{1}{r}{-}    & \multicolumn{1}{r}{-}   & \multicolumn{1}{r}{-}   & \multicolumn{1}{r}{-}                                                                   \\ \hline
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Time \\ series \\ classifier\\ (ours)\end{tabular}}} & KNN-DTW  & 0.99       & 1.00       & 1.00      &  & 1.00                     & 0.93                     & 0.97                     & 0.98                                                                &  & 0.79       & 1.00       & 0.88      &  & 1.00                     & 0.90                    & 0.95                    & \textbf{0.91}                                                                           \\
                                                                                                        & HMM      & 0.99       & 0.80       & 0.88      &  & 0.35                     & 0.96                     & 0.52                     & 0.70                                                                &  & 0.83       & 0.46       & 0.59      &  & 0.82                     & 0.97                    & 0.89                    & 0.74                                                                                    \\
                                                                                                        & TSF      & 1.00       & 1.00       & 1.00      &  & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & 1.00                                                                &  & 0.77       & 0.91       & 0.83      &  & 0.96                     & 0.90                    & 0.93                    & \textbf{0.88}                                                                           \\
                                                                                                        & TSBF     & 1.00       & 1.00       & 1.00      &  & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & 1.00                                                                &  & 0.69       & 0.82       & 0.75      &  & 0.93                     & 0.86                    & 0.89                    & 0.82                                                                                    \\
                                                                                                        & BOSSVS   & 1.00       & 1.00       & 1.00      &  & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & 1.00                                                                &  & 0.46       & 0.91       & 0.61      &  & 0.94                     & 0.59                    & 0.72                    & 0.67                                                                                    \\
                                                                                                        & SAX-VSM  & 1.00       & 1.00       & 1.00      &  & 0.98                     & 1.00                     & 0.99                     & 0.99                                                                &  & 0.27       & 0.64       & 0.38      &  & 0.71                     & 0.35                    & 0.47                    & 0.42                                                                                    \\ \hline
\end{tabular}
\end{table*}

==> tabs/res_training_set.tex <==
\begin{table}[tbhp]
\centering
\caption{Results of overfitting detection methods on the simulated dataset. (Prec: precision; Rec: recall; F-s: F-score; Avg F-s: macro average F-score)}
\label{tab:res_training_set}
\begin{tabular}{ll|rrr|lll|r}
\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{Detection method}}                                                             & \multicolumn{3}{c|}{Non-overfitting} & \multicolumn{3}{c|}{Overfitting}                                                & \multirow{2}{*}{\begin{tabular}[c]{@{}r@{}}Avg \\ F-s\end{tabular}} \\
\multicolumn{2}{l|}{}                                                                                              & Prec       & Rec        & F-s        & \multicolumn{1}{r}{Prec} & \multicolumn{1}{r}{Rec}  & \multicolumn{1}{r|}{F-s}  &                                                                     \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Correlation\\ based\end{tabular}}                            & Spearman & 0.99       & 1.00       & 0.99       & 0.95                     & 0.89                     & 0.92                      & \textbf{0.95}                                                       \\
                                                                                                        & Pearson  & 0.99       & 0.97       & 0.98       & 0.79                     & 0.93                     & 0.85                      & 0.92                                                                \\
                                                                                                         & Autocorr & 0.97       & 0.94       & 0.95       & 0.59                     & 0.73                     & 0.65                      & 0.80                                                                \\ \midrule
% PV                                                                                                      & PV       & 0.89       & 0.85       & 0.87       & 0.07                     & 0.09                     & 0.08                      & 0.47                                                                \\ 
% \midrule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Time \\ series \\ classifier\\ (ours)\end{tabular}}} & KNN-DTW  & 0.99       & 1.00       & 1.00       & 0.98                     & 0.93                     & 0.95                      & 0.97                                                                \\
                                                                                                        & HMM-GMM      & 0.95       & 0.55       & 0.70       & 0.16                     & 0.75                     & 0.27                      & 0.48                                                                \\
                                                                                                        & TSF      & 1.00       & 1.00       & 1.00       & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r|}{1.00} & \textbf{1.00}                                                       \\
                                                                                                        & TSBF     & 1.00       & 1.00       & 1.00       & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r|}{1.00} & \textbf{1.00}                                                       \\
                                                                                                        & BOSSVS   & 1.00       & 1.00       & 1.00       & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r}{1.00} & \multicolumn{1}{r|}{1.00} & \textbf{1.00}                                                       \\
                                                                                                        & SAX-VSM  & 0.99       & 1.00       & 0.99       & 0.98                     & 0.91                     & 0.94                      & 0.97                                                                \\ \bottomrule
\end{tabular}
\end{table}


==> tabs/sig_test_loss.tex <==

\begin{table*}[tbhp]
\centering
\caption{Significance testing results of the delays for overfitting prevention. (Ws.: Window size)}
\label{tab:sig_test_loss}
\begin{tabular}{lrrrr|lrrrr}
\toprule
Classifier &
  Ws. &
  P &
  \begin{tabular}[c]{@{}r@{}}Effect \\ Size\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Cliff's\\ d value\end{tabular} &
  Classifier &
  Ws. &
  P &
  \begin{tabular}[c]{@{}r@{}}Effect \\ Size\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Cliff's\\ d value\end{tabular} \\ \midrule
\multirow{5}{*}{BOSSVS}  & 20  & 0.000 & large  & -0.600 & \multirow{5}{*}{SAX-VSM} & 20  & 0.000 & large & -1.000 \\
                         & 40  & 0.001 & medium & -0.405 &                          & 40  & 0.000 & large & -0.956 \\
                         & 60  & 0.000 & large  & -0.476 &                          & 60  & 0.000 & large & -0.868 \\
                         & 80  & 0.000 & large  & -0.522 &                          & 80  & 0.000 & large & -0.817 \\
                         & 100 & 0.001 & medium & -0.449 &                          & 100 & 0.000 & large & -0.681 \\ \midrule
\multirow{5}{*}{HMM-GMM} & 20  & 0.000 & large  & -1.000 & \multirow{5}{*}{TSBF}    & 20  & 0.000 & large & -0.875 \\
                         & 40  & 0.000 & large  & -0.966 &                          & 40  & 0.000 & large & -0.893 \\
                         & 60  & 0.000 & large  & -0.859 &                          & 60  & 0.000 & large & -0.742 \\
                         & 80  & 0.000 & large  & -0.793 &                          & 80  & 0.000 & large & -0.748 \\
                         & 100 & 0.000 & large  & -0.633 &                          & 100 & 0.000 & large & -0.581 \\ \midrule
\multirow{5}{*}{KNN-DTW} & 20  & 0.101 & small  & 0.200  & \multirow{5}{*}{TSF}     & 20  & 0.000 & large & -0.525 \\
                         & 40  & 0.001 & medium & -0.392 &                          & 40  & 0.000 & large & -0.804 \\
                         & 60  & 0.000 & large  & -0.485 &                          & 60  & 0.000 & large & -0.700 \\
                         & 80  & 0.000 & large  & -0.541 &                          & 80  & 0.000 & large & -0.709 \\
                         & 100 & 0.000 & large  & -0.517 &                          & 100 & 0.000 & large & -0.619 \\ \bottomrule
\end{tabular}
\end{table*}


==> tabs/stop_delay_epoch_acc.tex <==

\begin{table}[tbhp]
\centering
\small
\captionof{table}{The median delay and significant testing of our overfitting prevention methods based on zero-one validation loss curves with different window sizes. (Ws.: Window size; Md.: Median delay)}
\label{tab:stop_delay_epoch_acc}
\begin{tabular}{@{}rlrrrr|lrrrr@{}}
\toprule
Ws. &
  Classifier &
  Md. &
  P &
  \begin{tabular}[c]{@{}r@{}}Effect\\ size\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Cliff's\\ d value\end{tabular} &
  Classifier &
  Md. &
  P &
  \begin{tabular}[c]{@{}r@{}}Effect\\ size\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Cliff's\\ d value\end{tabular} \\ \midrule
20  & \multirow{5}{*}{BOSSVS}  & 13.5 & 0.684 & neg    & -0.050 & \multirow{5}{*}{SAX-VSM} & 5.0  & 0.000 & large  & -0.950 \\
40  &                          & 46.0 & 0.109 & small  & 0.198  &                          & 5.5  & 0.000 & large  & -0.976 \\
60  &                          & 44.5 & 0.494 & neg    & -0.087 &                          & 11.5 & 0.000 & large  & -0.884 \\
80  &                          & 46.5 & 0.115 & small  & -0.202 &                          & 14.5 & 0.000 & large  & -0.806 \\
100 &                          & 49.5 & 0.029 & small  & -0.284 &                          & 26.5 & 0.000 & large  & -0.716 \\ \midrule
20  & \multirow{5}{*}{HMM-GMM} & 2.0  & 0.000 & large  & -0.850 & \multirow{5}{*}{TSBF}    & 7.5  & 0.000 & large  & -0.750 \\
40  &                          & 5.0  & 0.000 & large  & -0.739 &                          & 14.5 & 0.000 & large  & -0.867 \\
60  &                          & 8.0  & 0.000 & large  & -0.656 &                          & 27.0 & 0.000 & large  & -0.809 \\
80  &                          & 18.0 & 0.000 & large  & -0.719 &                          & 37.0 & 0.000 & large  & -0.708 \\
100 &                          & 46.5 & 0.001 & medium & -0.431 &                          & 45.0 & 0.000 & large  & -0.561 \\ \midrule
20  & \multirow{5}{*}{KNN-DTW} & 48.5 & 0.000 & large  & 0.650  & \multirow{5}{*}{TSF}     & 12.5 & 0.001 & medium & -0.400 \\
40  &                          & 44.0 & 0.027 & small  & 0.273  &                          & 24.0 & 0.000 & large  & -0.726 \\
60  &                          & 47.0 & 0.392 & neg    & -0.109 &                          & 31.0 & 0.000 & large  & -0.630 \\
80  &                          & 48.5 & 0.194 & small  & -0.166 &                          & 42.5 & 0.000 & large  & -0.596 \\
100 &                          & 56.5 & 0.024 & small  & -0.292 &                          & 47.0 & 0.000 & large  & -0.479 \\ \bottomrule
\end{tabular}
\end{table}


==> tabs/surveyed_papers.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}

\begin{xltabular}{\textwidth}
% { l s X s l }
{l
                              >{\hsize=0.17\hsize}X
                              >{\hsize=0.76\hsize}X
                              >{\hsize=0.1\hsize}X
                              >{\hsize=0.07\hsize}X}
\caption{Information about the surveyed papers.} \label{tab:survey} \\
% \toprule
% Paper &
%   Authors &
%   Title &
%   Venue &
%   Year \\ \midrule

\toprule \multicolumn{1}{l}{\#P} & \multicolumn{1}{l}{Authors} & \multicolumn{1}{l}{Title} & \multicolumn{1}{l}{Venue} & \multicolumn{1}{l}{Year} \\ \midrule 
\endfirsthead

\multicolumn{5}{c}%
{\tablename\ \thetable{} -- continued from previous page} \\
\toprule \multicolumn{1}{l}{\#P} & \multicolumn{1}{l}{Authors} & \multicolumn{1}{l}{Title} & \multicolumn{1}{l}{Venue} & \multicolumn{1}{l}{Year} \\ \midrule 
\endhead

\multicolumn{5}{r}{{Continued on next page}} \\ \midrule 
\endfoot

\hline
\endlastfoot
  
P1  & Belkin et al. & Overfitting or perfect fitting? risk bounds for classification and regression rules that interpolate.               & NeurIPS                 & 2018 \\
P2    & Chatterjee \& Mishchenko & Circuit-based intrinsic methods to detect overfitting.                                            & ICML    & 2020 \\
P3    & Chatterji \& Long        & Foolish crowds support benign overfitting.                                                        & JMLR    & 2022 \\
P4    & Chen et al.              & Robust overfitting may be mitigated by properly learned smoothening.                              & ICLR    & 2021 \\
P5    & d'Ascoli et al.          & Triple descent and the two kinds of overfitting: where \& why do they appear?                     & NeurIPS & 2020 \\
P6    & Feldman et al.           & The advantages of multiple classes for reducing overfitting from test set reuse.                  & ICML    & 2019 \\
P7    & Feldman et al.           & Open problem: how fast can a multiclass test set be overfit?                                      & COLT    & 2019 \\
P8  & Frei et al.   & Benign overfitting without linearity: neural network classifiers trained by gradient descent for noisy linear data. & COLT                    & 2022 \\
P9    & He et al.                & Sparse double descent: where network pruning aggravates overfitting.                              & ICML    & 2022 \\
P10   & Huang et al.             & Sparse progressive distillation: resolving overfitting under pretrain-and-finetune paradigm.      & ACL     & 2022 \\
P11   & Ju et al.                & Overfitting can be harmless for basis pursuit, but only to a degree.                              & NeurIPS & 2020 \\
P12   & Ju et al.                & On the generalization power of overfitted two-layer neural tangent kernel models.                 & ICML    & 2021 \\
P13   & Kim et al.               & Understanding catastrophic overfitting in single-step adversarial training.                       & AAAI    & 2021 \\
P14   & Koehler et al.           & Uniform convergence of interpolators: Gaussian width, norm bounds and benign overfitting.         & NeurIPS & 2021 \\
P15   & Liu et al.               & Overfitting the data: compact neural video delivery via content-aware feature modulation.         & ICCV    & 2021 \\
P16   & Mohammed \& Cawley       & Over-fitting in model selection with Gaussian process regression.                                 & ICML    & 2017 \\
P17   & Rice et al.              & Overfitting in adversarially robust deep learning.                                                & ICML    & 2020 \\
P18   & Roelofs et al.           & A meta-analysis of overfitting in machine learning.                                               & NeurIPS & 2019 \\
P19   & Rozendaal et al.         & Overfitting for fun and profit: instance-adaptive data compression.                               & ICLR    & 2021 \\
P20 & Russo \& Zou  & How much does your data exploration overfit? controlling bias via information usage.                                & IEEE Trans. Inf. Theory & 2020 \\
P21   & Sanyal et al.            & How benign is benign overfitting?                                                                 & ICLR    & 2021 \\
P22   & Shamir                   & The implicit bias of benign overfitting.                                                          & COLT    & 2022 \\
P23   & Singla et al.            & Low curvature activations reduce overfitting in adversarial training.                             & ICCV    & 2021 \\
P24   & Song et al.              & Observational overfitting in reinforcement learning.                                              & ICLR    & 2020 \\
P25   & Steck                    & Autoencoders that don't overfit towards the identity.                                             & NeurIPS & 2020 \\
P26   & Sun et al.               & meProp: sparsified back propagation for accelerated deep learning with reduced overfitting.       & ICML    & 2017 \\
P27   & Telgarsky                & Stochastic linear optimization never overfits with quadratically-bounded losses on general data.  & COLT    & 2022 \\
P28   & Wang et al.              & Benign overfitting in multiclass classification: all roads lead to interpolation.                 & NeurIPS & 2021 \\
P29   & Webster et al.           & Detecting overfitting of deep generative networks via latent recovery.                            & CVPR    & 2019 \\
P30   & Werpachowski et al.      & Detecting overfitting via adversarial examples.                                                   & NeurIPS & 2019 \\
P31   & Xu et al.                & Overfitting avoidance in tensor train factorization and completion: prior analysis and inference. & ICDM    & 2021 \\
P32   & Zhang \& Amini           & Label consistency in overfitted generalized k-means.                                              & NeurIPS & 2021 \\
P33   & Zhang et al.             & Why overfitting isn't always bad: retrofitting cross-lingual word embeddings to dictionaries.     & ACL     & 2020 \\ \bottomrule
\end{xltabular}


% \begin{xltabular}{\textwidth}{|l|X|l|l}
% \caption{A sample long table.} \label{tab:long} \\

% \hline \multicolumn{1}{|c|}{\textbf{First column}} & \multicolumn{1}{c|}{\textbf{Second column}} & \multicolumn{1}{c|}{\textbf{Third column}} \\ \hline 
% \endfirsthead

% \multicolumn{3}{c}%
% {\tablename\ \thetable{} -- continued from previous page} \\
% \hline \multicolumn{1}{|c|}{\textbf{First column}} & \multicolumn{1}{c|}{\textbf{Second column}} & \multicolumn{1}{c|}{\textbf{Third column}} \\ \hline 
% \endhead

% \hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
% \endfoot

% \hline
% \endlastfoot

% P1 &
%   Overfitting or perfect fitting? risk bounds for classification and regression rules that interpolate. &
%   NeurIPS &
%   2018 \\
% P2    & Circuit-based intrinsic methods to detect overfitting.                                            & ICML    & 2020 \\
% P3    & Foolish crowds support benign overfitting.                                                        & JMLR    & 2022 \\
% P4    & Robust overfitting may be mitigated by properly learned smoothening.                              & ICLR    & 2021 \\
% P5    & Triple descent and the two kinds of overfitting: where \& why do they appear?                     & NeurIPS & 2020 \\
% P6    & The advantages of multiple classes for reducing overfitting from test set reuse.                  & ICML    & 2019 \\
% P7    & Open problem: how fast can a multiclass test set be overfit?                                      & COLT    & 2019 \\
% P8 &
%   Benign overfitting without linearity: neural network classifiers trained by gradient descent for noisy linear data. &
%   COLT &
%   2022 \\
% P9    & Sparse double descent: where network pruning aggravates overfitting.                              & ICML    & 2022 \\
% P10   & Sparse progressive distillation: resolving overfitting under pretrain-and-finetune paradigm.      & ACL     & 2022 \\
% P11   & Overfitting can be harmless for basis pursuit, but only to a degree.                              & NeurIPS & 2020 \\
% P12   & On the generalization power of overfitted two-layer neural tangent kernel models.                 & ICML    & 2021 \\
% P13   & Understanding catastrophic overfitting in single-step adversarial training.                       & AAAI    & 2021 \\
% P14   & Uniform convergence of interpolators: Gaussian width, norm bounds and benign overfitting.         & NeurIPS & 2021 \\
% P15   & Overfitting the data: compact neural video delivery via content-aware feature modulation.         & ICCV    & 2021 \\
% P16   & Over-fitting in model selection with Gaussian process regression.                                 & ICML    & 2017 \\
% P17   & Overfitting in adversarially robust deep learning.                                                & ICML    & 2020 \\
% P18   & A meta-analysis of overfitting in machine learning.                                               & NeurIPS & 2019 \\
% P19   & Overfitting for fun and profit: instance-adaptive data compression.                               & ICLR    & 2021 \\
% P20 &
%   How much does your data exploration overfit? controlling bias via information usage. &
%   \begin{tabular}[c]{@{}l@{}}IEEE Trans. \\ Inf. Theory\end{tabular} &
%   2020 \\
% P21   & How benign is benign overfitting?                                                                 & ICLR    & 2021 \\
% P22   & The implicit bias of benign overfitting.                                                          & COLT    & 2022 \\
% P23   & Low curvature activations reduce overfitting in adversarial training.                             & ICCV    & 2021 \\
% P24   & Observational overfitting in reinforcement learning.                                              & ICLR    & 2020 \\
% P25   & Autoencoders that don't overfit towards the identity.                                             & NeurIPS & 2020 \\
% P26   & meProp: sparsified back propagation for accelerated deep learning with reduced overfitting.       & ICML    & 2017 \\
% P27   & Stochastic linear optimization never overfits with quadratically-bounded losses on general data.  & COLT    & 2022 \\
% P28   & Benign overfitting in multiclass classification: all roads lead to interpolation.                 & NeurIPS & 2021 \\
% P29   & Detecting overfitting of deep generative networks via latent recovery.                            & CVPR    & 2019 \\
% P30   & Detecting overfitting via adversarial examples.                                                   & NeurIPS & 2019 \\
% P31   & Overfitting avoidance in tensor train factorization and completion: prior analysis and inference. & ICDM    & 2021 \\
% P32   & Label consistency in overfitted generalized k-means.                                              & NeurIPS & 2021 \\
% P33   & Why overfitting isn't always bad: retrofitting cross-lingual word embeddings to dictionaries.     & ACL     & 2020 \\ \bottomrule
% \end{xltabular}
